Is Integer Linear Programming All You Need for Deletion Propagation? A Unified and Practical Approach for Generalized Deletion Propagation

Deletion Propagation (DP) refers to a family of database problems rooted in the classical view-update problem: how to propagate intended deletions in a view (query output) back to the source database while satisfying constraints and minimizing side effects. Although studied for over 40 years, DP variants, their complexities, and practical algorithms have been typically explored in isolation. This work presents a unified and generalized framework for DP with several key benefits: (1) It unifies and generalizes all previously known DP variants, effectively subsuming them within a broader class of problems, including new, well-motivated variants. (2) It comes with a practical and general-purpose algorithm that is ``coarse-grained instance-optimal'': it runs in PTIME for all known PTIME cases and can automatically exploit structural regularities in the data, i.e. it does not rely on hints about such regularities as part of the input. (3) It is complete: our framework handles all known DP variants in all settings (including those involving self-joins, unions, and bag semantics), and allows us to provide new complexity results. (4) It is easy to implement and, in many cases, outperforms prior variant-specific solutions, sometimes by orders of magnitude. We provide the first experimental results for several DP variants previously studied only in theory.

==> datalabmacros.tex <==



\usepackage{amsmath}
\usepackage{graphicx} %
\usepackage{url}
\usepackage{enumitem} %

\newcommand\bmmax{2} %
\usepackage{bm} %

\usepackage{upgreek} %
\usepackage{soul} %
\usepackage{bbding} %
\usepackage{pifont} %

\usepackage{listings} %

\usepackage{tabularx} %
\usepackage{booktabs} %
\usepackage{multirow}
\usepackage{hhline} %
\usepackage{diagbox}
\usepackage{pgfplotstable} %

\usepackage{colortbl}
\definecolor{dg}{cmyk}{0.60,0,0.88,0.27}	

\usepackage{booktabs}  %


\usepackage{easybmat} %

\usepackage{rotating}		%


\RequirePackage{etoolbox}	%
\newcommand{\iflabelexists}[3]{\ifcsundef{r@#1}{#3}{#2}}


\usepackage{tikz} %
\usetikzlibrary{matrix}
\usetikzlibrary{calc}
\usetikzlibrary{math}
\usetikzlibrary{positioning,chains,fit,shapes,calc}
\definecolor{myblue}{RGB}{80,80,160}
\definecolor{mygreen}{RGB}{80,160,80}

\usetikzlibrary{arrows,shapes,trees,backgrounds,automata}
\usetikzlibrary{decorations.markings}
\usepackage{tikzsymbols}



\usepackage{subcaption} %
\captionsetup[figure]{font+=small} %
\captionsetup[table]{font+=small} %

\captionsetup[figure]{aboveskip=5pt}		%
\captionsetup[figure]{belowskip=-5pt}
\captionsetup[subfigure]{aboveskip=0pt, belowskip=0pt}		%
\captionsetup[subfigure]{justification=centering}






\usepackage[ruled,noend,linesnumbered]{algorithm2e} %

\DontPrintSemicolon     %
\SetNlSty{}{}{}                %
\SetAlgoInsideSkip{smallskip}   %
\SetAlCapSkip{1.5mm}             %
\setlength{\algomargin}{1.5mm}    %
\SetInd{1.5mm}{1.5mm}             %

\SetAlFnt{\small}			%
\SetAlCapFnt{\small}		%
\SetAlCapNameFnt{\small}


\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\newtheorem{observation}{Observation}
\newtheorem{problem}{Problem}
\newtheorem{algo}{Algorithm}
\newtheorem{answer}{Answer}
\newtheorem{question}{Question}
\newtheorem{questionW}{Question}
\newtheorem{resultW}{Result}
\newtheorem{hypothesis}{Hypothesis}		


\theoremstyle{remark}
\newtheorem{proofintuition}{Proof Intuition}
\newtheorem*{proofintuition*}{Proof Intuition}

\newtheorem{intuition}{Intuition}
\newtheorem*{intuition*}{Intuition}

\renewenvironment{questionW}[1][]
{%
  {\textit{Question \arabic{questionW}#1.}
  \stepcounter{questionW}}%
}
{%
}
\setcounter{questionW}{1}

\renewenvironment{resultW}[1][]
{%
\par\noindent
  {\textbf{Result \arabic{resultW}#1.}
  \stepcounter{resultW}}%
  \begin{itshape}%
}%
{\end{itshape}
}
\setcounter{resultW}{1}




\newcommand{\todo}[1]{{{\color{red}{[Todo: #1]}}}} %
\newcommand{\note}[1]{{{\color{blue}{[#1]}}}} %
\newcommand{\wolf}[1]{{{\color{orange}{[\textbf{WG}: #1]}}}}
\newcommand{\neha}[1]{{{\color{blue}{[\textbf{NM}: #1]}}}}



\newcommand{\deprecate}[1]{{{\color{gray}{[#1]}}}} %
\newcommand{\out}[1]{{{\color{gray}{[#1]}}}} %


\newcommand{\later}[1]{{\color{blue}{[\textbf{LATER}: #1]}}} 	%
\renewcommand{\later}[1]{} 	%
\newcommand{\laterr}[1]{{{\color{blue}{}}}}



\newcommand{\hide}[1]{} 		%
\newcommand{\mkclean}{
    \renewcommand{\note}{\hide}
	\renewcommand{\wolf}{\hide}
	\renewcommand{\neha}{\hide}
	\renewcommand{\later}{\hide}
	\renewcommand{\laterr}{\hide}
	\renewcommand{\todo}{\hide}
    \renewcommand{\deprecate}{\hide}	
}









\usepackage[capitalise,nameinlink]{cleveref} %


\crefname{conjecture}{Conjecture}{Conjectures}
\Crefname{equation}{Eq.}{Eqs.}

\crefformat{equation}{(#2#1#3)}						%
\crefrangeformat{equation}{(#3#1#4) to~(#5#2#6)}
\crefmultiformat{equation}{(#2#1#3)}%
{ and~(#2#1#3)}{, (#2#1#3)}{ and~(#2#1#3)}






\AtEndPreamble{%
    \hypersetup{colorlinks,
      linkcolor=purple,
      citecolor=blue,
      urlcolor=ACMDarkBlue,
      filecolor=ACMDarkBlue}}










\usepackage{marginnote}
\newcommand{\rebuttal}[2]{\marginnote{\textbf{\textcolor{blue}{#1}}}{\color{blue}#2}}
\newcommand{\new}[1]{{\color{blue}{#1}}}
\newcommand{\revision}[1]{{{\color{blue}{#1}}}}


\usepackage{tcolorbox}		%
\tcbuselibrary{breakable,skins}		%


\tcbset{examplestyle/.style={
		enhanced jigsaw,	%
		colback=blue!08,	%
		colframe=blue!08,	%
		arc=0mm,
		boxrule=1pt,		%
		left=1mm,
		right=1mm,
		left skip=0mm,  %
		right skip=0mm, %
		top=1mm,		%
		bottom=1mm,		%
		breakable,		%
		parbox = false,		%
		before={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},		
		after={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},				
		bottomrule = 0mm,
		boxsep = 0mm,					%
		topsep at break=0pt,			%
		bottomsep at break=0pt,			%
		pad at break=0mm,
		pad before break=0mm,		
		pad after break=1mm,		
		bottomrule at break=0mm,
		toprule at break=0mm,		
		}}

\tcolorboxenvironment{example}{examplestyle}

\newtheoremstyle{abcd}%
  {}%
  {}%
  {\itshape}%
  {}%
  {\scshape}%
  {.}%
  {.5em}%
  {}%

\theoremstyle{abcd}
\newtheorem{example}{Example}





\tcbset{definitionstyle/.style={
		enhanced jigsaw,	%
		colback=gray!10,	%
		colframe=gray!10,	%
		arc=0mm,
		boxrule=1pt,		%
		left=1mm,
		right=1mm,
		left skip=0mm,  %
		right skip=0mm, %
		top=1mm,		%
		bottom=1mm,		%
		breakable,		%
		parbox = false,		%
		before={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},		
		after={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},				
		bottomrule = 0mm,
		boxsep = 0mm,					%
		topsep at break=0pt,			%
		bottomsep at break=0pt,			%
		pad at break=0mm,
		pad before break=0mm,		
		pad after break=1mm,		
		bottomrule at break=0mm,
		toprule at break=0mm,		
		}}

\tcolorboxenvironment{definition}{definitionstyle}



\tcbset{qrboxstyle/.style={
		enhanced jigsaw,	%
		colback=gray!20,
		colframe=gray!40,
		arc=0mm,
		boxrule=1pt,		%
		left=1pt,
		right=1pt,
		topsep at break=1mm,			%
		top=1pt,		%
		bottom=0mm,		%
		breakable,		%
		parbox = false		%
		}}


\newcommand{\resultbox}[1]{
\begin{tcolorbox}[
	enhanced jigsaw,		%
	colback=red!5,
	colframe=red!75!black,	
	arc=0mm,
	left skip=0mm,
	right skip=0mm,	
	left=0mm,
	topsep at break=1mm,			%
	right=0mm,
	top=0mm,
	bottom=0mm,		%
	breakable,		%
	parbox = false		%
]
\emph{#1}
\end{tcolorbox}
}


\newcounter{resultboxenv}

\newsavebox{\coloredbgbox}
\newenvironment{resultboxenv}{
	\begin{lrbox}{\coloredbgbox}
		\begin{minipage}{\dimexpr1\linewidth-2\fboxsep-2\fboxrule\relax}
			\refstepcounter{resultboxenv}
			\emph{Result \theresultboxenv.}
			\itshape
		}
  		{
		\end{minipage}
	\end{lrbox}
	\begin{center}
		\fcolorbox{black}{black!05}{\usebox{\coloredbgbox}}
	\end{center}
}






\renewcommand\dbltopfraction{1} %
\setcounter{dbltopnumber}{3}	%






\RequirePackage{scalerel}
\RequirePackage{tikz}
\usetikzlibrary{svg.path}

\definecolor{orcidlogocol}{HTML}{A6CE39}
\tikzset{
  orcidlogo/.pic={
    \fill[orcidlogocol] svg{M256,128c0,70.7-57.3,128-128,128C57.3,256,0,198.7,0,128C0,57.3,57.3,0,128,0C198.7,0,256,57.3,256,128z};
    \fill[white] svg{M86.3,186.2H70.9V79.1h15.4v48.4V186.2z}
                 svg{M108.9,79.1h41.6c39.6,0,57,28.3,57,53.6c0,27.5-21.5,53.6-56.8,53.6h-41.8V79.1z M124.3,172.4h24.5c34.9,0,42.9-26.5,42.9-39.7c0-21.5-13.7-39.7-43.7-39.7h-23.7V172.4z}
                 svg{M88.7,56.8c0,5.5-4.5,10.1-10.1,10.1c-5.6,0-10.1-4.6-10.1-10.1c0-5.6,4.5-10.1,10.1-10.1C84.2,46.7,88.7,51.3,88.7,56.8z};
  }
}

\RequirePackage{etoolbox}
\DeclareRobustCommand\orcidicon[1]{\href{https://orcid.org/#1}{\mbox{\scalerel*{
\begin{tikzpicture}[yscale=-1, transform shape]
    \pic{orcidlogo};
\end{tikzpicture}
}{|}}}}
 
 
 
 
 

\usepackage{adjustbox}
\def\eox{\unskip\kern 10pt{\unitlength1pt\linethickness{.4pt}$\diamondsuit${}}}   



\makeatletter
\DeclareRobustCommand*\uell{\mathpalette\@uell\relax}
\newcommand*\@uell[2]{
  \setbox0=\hbox{$#1\ell$}
  \setbox1=\hbox{\rotatebox{10}{$#1\ell$}}
  \dimen0=\wd0 \advance\dimen0 by -\wd1 \divide\dimen0 by 2
  \mathord{\lower 0.1ex \hbox{\kern\dimen0\unhbox1\kern\dimen0}}
}
\makeatother

















\newcommand{\smallsection}[1]{\vspace{2mm}\noindent\textbf{#1.}} %
\newcommand{\introparagraph}[1]{\textbf{#1.}} %

\newcommand{\ourmethod}{\textsc{OurMethod}\xspace}
\renewcommand{\epsilon}{\varepsilon} %
\newcommand{\set}[1]{\{#1\}}                    %
\newcommand{\setof}[2]{\{{#1}\mid{#2}\}}        %

\newcommand{\define}{\stackrel{\textup{\tiny def}}{=}}

\newcommand{\datarule}{{\,:\!\!-\,}} %
\renewcommand{\vec}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\transpose}{\intercal}	%

\newcommand{\N}{\mathbb{N}} %
\newcommand{\R}{{\mathbb{R}}} %
\newcommand{\bigO}{{\mathcal{O}}} %
\renewcommand{\O}{{\mathcal{O}}} %
\renewcommand{\P}{{\mathbb{P}}} %
\newcommand{\PP}[1]{\mathbb{P} [ #1 ]} %
\newcommand{\E}{\mathbb{E}}
\newcommand{\sql}[1]{\textup{\textsf{\small#1}}}
\newcommand{\datastyle}[1]{\texttt{#1}}

\newcommand{\attr}{\texttt{attr}}
\newcommand{\head}{\texttt{head}}
\newcommand{\rels}{\texttt{rels}}

\DeclareMathOperator*{\argmin}{argmin}

\newcommand{\dom}{\texttt{dom}}
\newcommand{\EVar}{\textup{\texttt{EVar}}}  	
\newcommand{\at}{\textup{\texttt{at}}}  		
\newcommand{\fact}{\mathtt{FACT}} 
\newcommand{\minfact}{\mathtt{minFACT}} 
\newcommand{\Var}{\textup{\texttt{var}}}
\newcommand{\len}{\textup{\texttt{len}}}
\newcommand{\ptime}{$\mathsf{PTIME}$} 

\newcommand{\gdp}{\mathtt{GDP}}
\newcommand{\gdpilp}{\mathtt{ILP}[\gdp]} 
\newcommand{\gdpilpmiddle}{\mathtt{ILP}[\gdp\texttt{-2}]} 
\newcommand{\gdplp}{\mathtt{LP}[\gdp]} 
\newcommand{\gdpilpparam}[1]{\mathtt{ILP}[\gdp(#1)]}
\newcommand{\gdpilpbasic}{\mathtt{ILP_N}[\gdp]}
\newcommand{\gdpilpwildcard}{\mathtt{ILP_W}[\gdp]} 
\newcommand{\gdpilpsmooth}{\mathtt{ILP_S}[\gdp]} 


\newcommand{\dpvs}{\mathtt{DP\textsf{-}VS}}
\newcommand{\gdpdpvs}{\gdp_{\dpvs}}
\newcommand{\gdpdpvsilp}{\mathtt{ILP}[\gdpdpvs]}
\newcommand{\gdpdpvslp}{\mathtt{LP}[\gdpdpvs]}
\newcommand{\gdpdpvsilpparam}[1]{\mathtt{ILP}[\gdpdpvs(#1)]}
\newcommand{\gdpdpvslpparam}[1]{\mathtt{LP}[\gdpdpvs(#1)]}

\newcommand{\dpss}{\mathtt{DP\textsf{-}SS}}
\newcommand{\gdpdpss}{\gdp_{\dpss}}
\newcommand{\gdpdpssilp}{\mathtt{ILP}[\gdpdpss]}
\newcommand{\gdpdpsslp}{\mathtt{LP}[\gdpdpss]}
\newcommand{\gdpdpssilpparam}[1]{\mathtt{ILP}[\gdpdpss(#1)]}
\newcommand{\gdpdpsslpparam}[1]{\mathtt{LP}[\gdpdpss(#1)]}

\newcommand{\swp}{\mathtt{SWP}}
\newcommand{\gdpswp}{\gdp_{\swp}}
\newcommand{\gdpswpilp}{\mathtt{ILP}[\gdpswp]}
\newcommand{\gdpswplp}{\mathtt{LP}[\gdpswp]}
\newcommand{\gdpswpilpparam}[1]{\mathtt{ILP}[\gdpswp(#1)]}
\newcommand{\gdpswplpparam}[1]{\mathtt{LP}[\gdpswp(#1)]}

\newcommand{\adp}{\mathtt{ADP\textsf{-}SS}}
\newcommand{\gdpadp}{\gdp_{\adp}}
\newcommand{\gdpadpilp}{\mathtt{ILP}[\gdpadp]}
\newcommand{\gdpadplp}{\mathtt{LP}[\adp]}
\newcommand{\gdpadplpparam}[1]{\mathtt{LP}[\gdpadp(#1)]}
\newcommand{\adpspl}{\mathtt{ADP\texttt{-}S}}
\newcommand{\dpvsspl}{\mathtt{DPVS\texttt{-}S}}
\newcommand{\swpspl}{\mathtt{SWP\texttt{-}S}}


\newcommand{\resilp}{\mathtt{ILP}[\resdecision^*]} 
\newcommand{\resilpparam}[1]{\mathtt{ILP}[\resdecision^*({#1})]}
\newcommand{\reslp}{\mathtt{LP}[\resdecision^*]}
\newcommand{\reslpparam}[1]{\mathtt{LP}[\resdecision^*({#1})]} 
\newcommand{\rspilp}{\mathtt{ILP}[\rspdecision^*]}
\newcommand{\rspilpparam}[1]{\mathtt{ILP}[\rspdecision^*({#1})]}
\newcommand{\rsplp}{\mathtt{LP}[\rspdecision^*]}
\newcommand{\rsplpparam}[1]{\mathtt{LP}[\rspdecision^*({#1})]}
\newcommand{\rspmilp}{\mathtt{MILP}[\rspdecision^*]}
\newcommand{\rspmilpparam}[1]{\mathtt{MILP}[\rspdecision^*({#1})]}

\newcommand{\viewdel}{\mathcal{V}_{\texttt{del}}}
\newcommand{\viewpres}{\mathcal{V}_{\texttt{pres}}}
\newcommand{\viewmax}{\mathcal{V}_{\texttt{max}}}
\newcommand{\viewmin}{\mathcal{V}_{\texttt{min}}}
\newcommand{\viewdeli}{V_{\texttt{del}}^i}
\newcommand{\viewpresi}{V_{\texttt{pres}}^i}
\newcommand{\viewmaxi}{V_{\texttt{max}}^i}
\newcommand{\viewmini}{V_{\texttt{min}}^i}

\newcommand{\querydel}{\mathcal{Q}_{\texttt{del}}}
\newcommand{\querypres}{\mathcal{Q}_{\texttt{pres}}}
\newcommand{\querymax}{\mathcal{Q}_{\texttt{max}}}
\newcommand{\querymin}{\mathcal{Q}_{\texttt{min}}}

\newcommand{\querydelparam}[1]{{Q}_{\texttt{del}}^{#1}}
\newcommand{\querypresparam}[1]{{Q}_{\texttt{pres}}^{#1}}
\newcommand{\querymaxparam}[1]{{Q}_{\texttt{max}}^{#1}}
\newcommand{\queryminparam}[1]{{Q}_{\texttt{min}}^{#1}}


\newcommand{\kdel}{\vec k_{\texttt{del}}}
\newcommand{\kpres}{\vec k_{\texttt{pres}}}
\newcommand{\kdelparam}[1]{k_{\texttt{del}}^{#1}}
\newcommand{\kpresparam}[1]{k_{\texttt{pres}}^{#1}}


\newcommand{\ijpdlp}{\mathtt{DLP[\res\mathtt{IJP}]}}
\newcommand{\ijpdlpparam}[1]{\mathtt{DLP}[\res\mathtt{IJP}({#1})]}

\newcommand{\res}{\mathtt{RES}}
\newcommand{\resdecision}{\mathtt{RES}}
\newcommand{\rspdecision}{\mathtt{RSP}}
\newcommand{\source}{\mathtt{DP_{source}}} 
\newcommand{\PTIME}{\textup{\textsf{PTIME}}\xspace} 
\newcommand{\NPC}{\textup{\textsf{NPC}}\xspace} 
\newcommand{\exoset}{E}

\newcommand{\opt}{\sql{OPT}\xspace}			%
\newcommand{\occ}{\mathrm{occ}}
\newcommand*\conj[1]{\bar{#1}}
\newcommand{\Lineage}{\textup{\texttt{Lin}}}  	
\newcommand{\Provenance}{\textup{\texttt{Prov}}}  	
\newcommand{\NP}{\textup{\textsf{NP}}\xspace}
\newcommand{\HVar}{\textup{\texttt{HVar}}} 		

\newcommand{\ADom}{{\mathit{ADom}}} 

\newcommand{\SepVar}{\textup{\texttt{SepVar}}}  	
\newcommand{\projpd}[1]{\pi^p_{#1}}
\newcommand{\projp}[1]{\pi^p_{\!-\!#1}}
\newcommand{\joinp}[2]{\Join^p\!\! \big[#2\big]}
\newcommand{\score}{\textit{score}}  
\newcommand{\join}[2]{\Join\!\! \big(#2\big)}
\newcommand{\proj}[1]{\pi_{\!-\!#1}}
\newcommand{\projd}[1]{\pi_{#1}}

\newcommand{\var}{\textup{\texttt{var}}}      	

\newcommand{\true}{\texttt{true}\xspace}		
\newcommand{\false}{\texttt{false}\xspace}	
\newcommand{\bigset}[2]{\bigl\{ #1 \,\bigm|\, #2 \bigr\} }

\newcommand{\Count}{\texttt{count}}

\newcommand{\sat}{\mbox{{\rm\sc SAT}}}

\newcommand{\w}{{\vec w}}      	


\newcounter{myeqn}
\newcommand{\myequation}[2]{\par\refstepcounter{theorem}
\setcounter{myeqn}{\value{theorem}}\vspace{4mm}\label{#1}
\noindent\makebox[\linewidth]{\hfill${\displaystyle #2 }$\hfill
{\mbox{\rm (\ref{#1})}}}
\par\smallskip\vspace{2mm}}






\newcommand{\enSymb}{\textup{n}}
\newcommand{\exSymb}{\textup{x}}
\newcommand{\en}[1]{{#1}^{\enSymb}}	
\newcommand{\ex}[1]{{#1}^{\exSymb}}



\usepackage{xspace}            %

\newcommand{\sign}{\texttt{sign}\xspace}		%
\newcommand{\col}{\textrm{col}\xspace}		%
\newcommand{\witness}{\texttt{witness}\xspace}		%
\newcommand{\witnesses}{\texttt{witnesses}\xspace}		%
\newcommand{\arity}{\textsf{arity}\xspace}		%
\newcommand{\Adom}{\textup{\textit{Adom}}}		%
\newcommand{\TID}{\textit{TID}}
\newcommand{\indb}{\textit{indb}}


\newcommand{\chain}{q_{\textup{\textrm{chain}}}} 
\newcommand{\np}{\mbox{{\rm NP}}}
\newcommand{\Tri}{\textup{\textrm{T}}} 
\newcommand{\vc}{q_{\textup{\textrm{vc}}}} 
\newcommand{\rats}{q_{\textup{\textrm{rats}}}}  
\newcommand{\lin}{q_{\textup{\textrm{lin}}}} 
\newcommand{\p}{\mbox{{\rm P}}}

\newcommand{\sprout}{{\tt SPROUT}\xspace}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\PPP}{{{\mathbb{P}}}}       
\newcommand{\vars}[1]{\text{\sl vars}(#1)}

\newcommand{\DNF}{{{\mathrm{DNF}}}}       
\newcommand{\outdeg}{{{\mathrm{out}}}}
\newcommand{\indeg}{{{\mathrm{in}}}}
\newcommand{\veo}{\mathtt{veo}}
\newcommand{\mveo}{\mathtt{mveo}}
\newcommand{\PV}{\mathit{PV}}
\newcommand{\QPV}{\mathit{QPV}}
\newcommand{\PVF}{\mathit{PVF}}
\newcommand{\wt}{c}

\renewcommand{\S}{\mathcal{S}}
\newcommand{\T}{\mathcal{T}}



\newcommand{\qkchain}{Q_{k}^\infty}
\newcommand{\qkcycle}{Q_{k}^\circ}
\newcommand{\qkstar}{Q_{k}^\star}
\newcommand{\qtwochain}{Q_{2}^\infty}
\newcommand{\qthreechain}{Q_{3}^\infty}
\newcommand{\qfourchain}{Q_{4}^\infty}
\newcommand{\qfivechain}{Q_{5}^\infty}
\newcommand{\qfivecycle}{Q_{5}^\circ}
\newcommand{\qthreestar}{Q_{3}^\star}
\newcommand{\qtwostar}{Q_{2}^\star}
\newcommand{\qtriangle}{Q^\triangle}
\newcommand{\qtriangleunary}{Q_{A}^{\triangle}}
\newcommand{\qtrianglebinary}{Q_{AB}^{\triangle}}
\newcommand{\qtwochainwe}{Q_{2\mathit{WE}}^\infty}
\newcommand{\qsixcyclewe}{Q_{6\mathit{WE}}^\circ}
\newcommand{\qsjtwochain}{Q_{2-\mathit{SJ}}^\infty}
\newcommand{\qsjtwoconf}{Q_{2-\mathit{SJ}}^\sim}
\newcommand{\qsjzsix}{Q_{\mathit{SJ}}^\texttt{z6}}
\newcommand{\qsjtriangletwochain}{Q^{\triangle\texttt{-}}}
\newcommand{\qthreeray}{Q^{3*}}
\newcommand{\qfourray}{Q^{4*}}
\newcommand{\qfiveray}{Q^{5*}}
\newcommand{\qsixray}{Q^{6*}}


\definecolor{dg}{cmyk}{0.60,0,0.88,0.27}

\renewcommand{\deg}{\mathrm{d}}


\renewcommand{\angle}[1]{ \langle #1 \rangle }


\newcommand{\highlight}[1]{ {\color{Red}{#1}} }		%

\newcommand{\IS}{\textrm{IndSet}}	

\newcommand{\plans}{\mathrm{plans}}

\usepackage{graphbox} %

\usetikzlibrary{tikzmark, calc}
\usetikzlibrary{arrows.meta,arrows}
\tikzset{
    double color fill/.code 2 args={
        \pgfdeclareverticalshading[%
            tikz@axis@top,tikz@axis@middle,tikz@axis@bottom%
        ]{diagonalfill}{100bp}{%
            color(0bp)=(tikz@axis@bottom);
            color(50bp)=(tikz@axis@bottom);
            color(50bp)=(tikz@axis@middle);
            color(50bp)=(tikz@axis@top);
            color(100bp)=(tikz@axis@top)
        }
        \tikzset{shade, left color=#1, right color=#2, shading=diagonalfill}
    }
}
\newcommand\BGcell[4][0pt]{%
  \begin{tikzpicture}[overlay,remember picture]%
    \path[#4] ( $ (pic cs:#2) + (-.5\tabcolsep,1.9ex) $ ) rectangle ( $ (pic cs:#3) + (\tabcolsep,-#1*\baselineskip-.8ex) $ );
  \end{tikzpicture}%
}%
\newcounter{BGnum}
\setcounter{BGnum}{1}
\newcommand\cellBG[3]{
    \multicolumn{1}{
        !{\BGcell{startBG\arabic{BGnum}}{endBG\arabic{BGnum}}{%
                #1}
            \tikzmark{startBG\arabic{BGnum}}}
            #2
        !{\tikzmark{endBG\arabic{BGnum}}}}
        {#3} 
      \addtocounter{BGnum}{1}
}

\usepackage{dcolumn, array, booktabs}
\newcolumntype{.}{D{.}{.}{-1}}
\newcommand*{\tabhead}[1]{\multicolumn{1}{c}{#1}}

\newtheoremstyle{dotless}{}{}{\itshape}{}{\bfseries}{}{ }{}
\theoremstyle{dotless}
\newtheorem*{specialexamplenotitle*}{}

\raggedbottom


\usepackage{thmtools}
\usepackage{thm-restate} 

\newcommand{\x}  { \mathrm{x}}			%


\usepackage{listings}

\lstset{
  basicstyle=\ttfamily,
  keywordstyle=\color{blue},
  stringstyle=\color{red},
  commentstyle=\color{blue},
  showstringspaces=false,
  breaklines=true,
  captionpos=b,
  numberstyle=\tiny\color{gray},
  frame=single,
  morecomment=[l]{\%}
}

\usepackage{xurl}

\newcommand{\colorcirc}[2]{\protect\raisebox{-0.5pt}{\protect\tikz{\protect\path
[fill=#1] (0,0.004) circle [radius=0.135];\protect\node [inner sep=0,outer
sep=0, font=\sffamily, scale=0.9] at (0,0) {\textbf{\textcolor{white}{\small{#2}}}};}}}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,fill=black,draw,text=white, inner sep=0.7pt] (char) 
			{#1};}} 			

\newcommand*\circledwhite[1]{\tikz[baseline=(char.base)]{
			\node[shape=circle,fill=white,draw,text=black,inner sep=0.7pt] (char) {#1};}} 			


\usepackage{breqn}


